Remember What You Want to Forget: Algorithms for Machine Unlearning

We study the problem of unlearning datapoints from a learnt model. The learner first receives a dataset $S$ drawn i.i.d. from an unknown distribution, and outputs a model $\widehat{w}$ that performs well on unseen samples from the same distribution. However, at some point in the future, any training datapoint $z \in S$ can request to be unlearned, thus prompting the learner to modify its output model while still ensuring the same accuracy guarantees. We initiate a rigorous study of generalization in machine unlearning, where the goal is to perform well on previously unseen datapoints. Our focus is on both computational and storage complexity. For the setting of convex losses, we provide an unlearning algorithm that can unlearn up to $O(n/d^{1/4})$ samples, where $d$ is the problem dimension. In comparison, in general, differentially private learning (which implies unlearning) only guarantees deletion of $O(n/d^{1/2})$ samples. This demonstrates a novel separation between differential privacy and machine unlearning.

==> files/lower-gaussian.tex <==
Consider the following mean estimation problem.
Let $\mu$ be u.a.r. chosen from $\{-a, a\}$. Let $V\sim N(\mu, \sigma_m^2)$ and $X_1, \ldots, X_{n_2}$ are i.i.d. samples from $N(\mu, 1)$. The following is a lower bound on the mean squared error of any estimate $\hat \mu$ of $\mu$ using $V$ and $X_1, \ldots, X_{n_2}$.

\begin{lemma}
For any $\hat \mu$, 
\begin{align}
\expect{(\hat \mu-\mu)^2}\ge \frac1{32} \min\left\{\sigma_m^2, \frac{1}{n_2}\right\}.
\end{align}
\end{lemma} 
\begin{proof}
Let $Z=(V, X_1, \ldots, X_{n_2})$. Then, using the fact that the coordinates of $Z$ are independent given $\mu$ and by the additivity of divergence for independent random variables we obtain
\begin{align}
D(Z|\mu=a\|Z|\mu=-a) = \frac{4a^2}{\sigma_m^2}+ n_2 \cdot {4a^2}.
\end{align}  
By Pinsker's inequality, 
\begin{align}
d_{\rm TV}(Z|\mu=a,Z|\mu=-a)
&\le \frac1{\sqrt 2} \left(\frac{4a^2}{\sigma_m^2}+ n_2 \cdot {4a^2}\right)^{1/2}\nonumber\\
&\le{\frac{a}{\sigma_m}} +{a\sqrt{n_2}}.
\end{align}
If $a = 0.25\cdot \min\{\sigma_m, 1/\sqrt{n_2}\}$, then  ${\frac{a}{\sigma_m}} +{a\sqrt{n_2}}<0.5$. By Le Cam's two point method, 
\begin{align}
\expect{(\hat \mu-\mu)^2}\ge 0.5\cdot a^2 = \frac1{32}\cdot \left\{\sigma_m^2, \frac{1}{n_2}\right\}
\end{align}
\end{proof}



==> files/unlearning_convex.tex <==
In this section, we provide learning and unlearning algorithms when
the loss function $f(\cdot, z)$ is convex. In particular, we assume that $f$ satisfies: 
\begin{assumption}
\label{ass:f_properties} 
For any $z \in \cZ$, the function $f(w, z)$ is convex, $L$-Lipschitz
and $M$-Hessian Lipschitz in $w$.
\end{assumption} 

We first give unlearning algorithms under the additional assumption
that the function $f$ is $\lambda$-strongly convex. We then provide
unlearning algorithms for convex losses by appealing to the strongly convex case
after adding regularization. Finally, throughout the section, we will assume that the domain $\cW = \bbR^d$. 


\subsection{Strongly convex loss}  \label{sec:sc_loss} 
Our learning and unlearning are denoted by $A_{sc}$ and $\bar{A}_{sc}$
, and are given in \pref{alg:learningalg_rerm_sco}
and \pref{alg:unlearningalg_rerm_sco} respectively. When given a dataset $S$ of $n$ points sampled iid from a distribution
$\cD$, the learning algorithm $A_{sc}$ returns the point $\wh w$ which
minimizes the empirical loss, i.e. the $\wh
w \in \argmin_{w \in \cW} \wh F(w)$, where $\wh
F(w) \ldef{} \frac{1}{n} \sum_{z \in S} f(w, z)$ and also $T(S)$ that
contains the Hessian of the empirical loss $\wh F(w)$ evaluated at the
point $\wh w$, i.e. $T(S) = \crl{ \grad^2 \wh F(\wh w)}$.

The unlearning algorithm $\bar{A}_{sc}$ receives as input the set of
delete requests $U$, the point $\wh w$ and the data summary
$T(S)$. % The data summary $T(S)$
The algorithm first estimates the
matrix $\wh H$, which denotes the Hessian of the empirical function on
the dataset $S \setminus U$ when evaluated at the point $\wh w$. $\wh H$ is computed by removing the
Hessian of the samples in $U$ from the Hessian of the empirical loss
on $S$ received in $T(S)$ (see \pref{line:gradient_estimation}). After
computing $\wh H$, $\bar{A}_{sc}$ computes the point
$\bar{w}$ by removing the contribution of the deleted points $U$ from
$\wh w$ as:
\begin{align*}
\bar{w} = \wh w +  \frac{1}{n - m} \prn{\wh H}^{-1} \sum_{z \in U} \grad f(\wh w, z). \numberthis \label{eq:pass1}
\end{align*}
Finally, $\bar{A}_{sc}$ perturbs the point $\bar{w}$ with noise $\nu$ drawn from $\cN(0, \sigma^2 \bbI_d)$ and returns the perturbed point $\wt w$. 

\begin{algorithm}[tb]
\caption{Learning algorithm ($A_{sc}$)} 
\begin{algorithmic}[1]
   \Require Dataset $S: \crl*{z_i}_{i=1}^{n} \sim \cD^{n}$, loss function: $f$. 
   \State Compute $$\wh w \leftarrow \argmin_{w} ~ \wh F (w) \ldef{} \frac{1}{n} \sum_{i=1}^{n} f(w, z_i).$$
   \State \textbf{return} $\prn{\wh w, \grad^2 \wh F(\wh w)}$.  
\end{algorithmic} 
\label{alg:learningalg_rerm_sco}  
\end{algorithm} 
\begin{algorithm}[tb] 
\caption{Unlearning algorithm ($\bar{A}_{sc}$)} 
\begin{algorithmic}[1]
   \Require Delete requests: $U = \crl*{z_j}_{j=1}^{m} \subseteq S$, output of $A_{sc}(S)$: $\wh w$, additional statistic $T(S): \crl{\grad^2 \wh F(\wh w)}$, loss function: $f(w, z)$. 
   \State Set $\gamma = \frac{2Mm^2 L^2}{\lambda^3 n^2}$, $\sigma = \frac{\gamma}{\epsilon} \sqrt{2 \ln(1.25 / \delta)}.$ 
   \State\label{line:gradient_estimation}Compute $$\wh H = \frac{1}{n-m} \prn{n \grad^2 \wh F(\wh w) - \sum_{z \in U} \grad^2 f(\wh w, z)}.$$
   \State Define $$\bar{w} \ldef{} \wh w +  \frac{1}{n - m} \prn{\wh H}^{-1} \sum_{z \in U} \grad f(\wh w, u).$$ 
   \State Sample $\nu \in \bbR^d$ from $\cN(0, \sigma^2 \bbI_d)$. 
   \State \textbf{return} $\wt w \ldef \bar{w}  +  \nu$.  \end{algorithmic}  
\label{alg:unlearningalg_rerm_sco}  
\end{algorithm} 


In the following, we prove bounds on the excess population risk for the output $\wh w$ of the algorithm $A_{sc}$, and the output $\wt w$ of the algorithm $\bar{A}_{sc}$. We will also show that $A_{sc}$ and $\bar{A}_{sc}$ are $(\epsilon, \delta)$-forgetting. Our main insight that leads to improvements in deletion capacity over differential privacy is the following technical lemma. \pref{lem:w_update_v_main}  suggests that for well behaved loss functions $f(w, z)$, when deleting $m$ samples, we can approximate the empirical minimizer on the dataset $S \setminus U$ upto a precision of $O(m^2 / n^2)$ by the point $\bar{w}$ computed in \pref{eq:pass1}. This implies that the standard deviation for noise needs to scales as $\sigma \propto O(m^2 / n^2)$, that is smaller than the amount of noise typically added for DP learning \citep{dwork2014algorithmic} by a quadratic factor. 
\begin{lemma} 
\label{lem:w_update_v_main} 
Let $f(w, z)$ satisfy \pref{ass:f_properties}. For any dataset $S$ of $n$ samples $\crl{z_i}_{i=1}^n$ and a set $U \subseteq S$ of $m$, let the points $\wh w$ and $\wh w'$ be defined as: 
\begin{align*} 
&\wh w \ldef{} \argmin_{w}  \frac{1}{n} \sum_{z \in S} f(w, z) \qquad \text{and}  \\ &{\wh w'} \ldef{}  \argmin_{w}  \frac{1}{n - m} \sum_{z \in S \setminus U} f(w, z).  
\end{align*}Then, the points ${\wh w}$ and $\wh w'$ satisfy
\begin{align*} 
\nrm[\Big]{\wh w' - \wh w -  \frac{1}{n - m} \prn{\wh H}^{-1} \sum_{z \in u} \grad f(\wh w, z)} \leq \frac{2 M m^2 L^2}{\lambda^3 n^2}, 
\end{align*} where the matrix $\wh H \ldef{} \frac{1}{n -m} \sum_{z \in S \setminus U} \grad^2 f(\wh w, z)$.  
\end{lemma} 
 
We defer the proof to the Appendix. In the following, we show that the learning algorithm $A_{sc}$ and the unlearning algorithm $\bar{A}_{sc}$ is $(\epsilon, \delta)$-forgetting. 

\begin{lemma}[Forgetting guarantee] 
\label{lem:dp_guarantee} For any distribution $\cD$, dataset $S \sim \cD^n$, $U \subseteq S$, the algorithms $A_{sc}$ and $\bar{A}_{sc}$ satisfy the following guarantees for any set $W \subseteq \bbR^d$, 
\arxiv{\begin{enumerate}[label=(\alph*)]
\item $\Pr \prn{\bar{A}_{sc}(U, A_{sc}(S), T(S)) \in W} \leq e^\epsilon \Pr \prn{\bar{A}_{cs}(\emptyset, A_{sc}(S \setminus U), T(S \setminus U)) \in W} + \delta$, and 
\item  $\Pr \prn{\bar{A}_{sc}(\emptyset, A_{sc}(S \setminus U), T(S\setminus U)) \in W} \leq e^\epsilon \Pr \prn{\bar{A}_{sc}(U, A_{sc}(S), T(S)) \in W} + \delta$. 
\end{enumerate}  
}
\icml{\begin{enumerate}[label=(\alph*)]
\item $\Pr \prn{\bar{A}_{c}(U, A_{c}(S), T(S)) \in W} $ \\ $\leq e^\epsilon \Pr \prn{\bar{A}_{c}(\emptyset, A_{c}(S \setminus U), T(S \setminus U)) \in W} + \delta$, and 
\item  $\Pr \prn{\bar{A}_{c}(\emptyset, A_{c}(S \setminus U), T(S\setminus U)) \in W}$\\ $\leq e^\epsilon \Pr \prn{\bar{A}_{c}(U, A_{c}(S), T(S)) \in W} + \delta$. 
\end{enumerate}}
\end{lemma}
\begin{proof}  
  The follow proof follows along the lines of the proof of the differential privacy guarantee for the Gaussian mechanism (see, e.g.,  \citep[Appendix A]{DworkR14}).  Recall that  $\wh w = A(S)$, and let $\bar{w}$ be the local variable defined in \pref{alg:unlearningalg_rerm_sco} in order to compute the point $\wt w$. By definition, 
\begin{align*}
\bar{w} = \wh w +  \frac{1}{n - m} \prn{\wh H}^{-1} \grad f(\wh w, z). \numberthis \label{eq:dp_guarantee1} 
\end{align*}

Further, let $\wh w'$ denote the output of the learning algorithm $A_{sc}$ when trained on the dataset $S \setminus U$, i.e. $\wh w' = A(S \setminus U)$. Similarly, let $\wt w'$ denote the output of our unlearning algorithm $\bar{A}_{sc}$ and $\bar{w}'$ denote the corresponding local variable in this case, when we request $\emptyset$ points to be deleted. Specifically, $\wh w'_1 = \bar{A}_{sc}(\emptyset, A(S \setminus U))$ and, by construction, $\bar{w}' = \wh w'$. Recall that 

%Since, the algorithm $A_{sc}$ returns the minimizer of the empirical loss on the returned dataset, we note that 
\begin{align*}
&\wh w \ldef{} A(S) =  \argmin_{w} \frac{1}{n} \sum_{z \in S} f(w, z). 
\intertext{and that} 
&\wh w' \ldef{} A(S \setminus U) =  \argmin_{w} \frac{1}{n - m} \sum_{z \in S \setminus U} f(w, z). 
\end{align*}
An application of \pref{lem:w_update_v_main} implies that 
\begin{align*}
\nrm[\Big]{\wh w'  - \wh w -  \frac{1}{n - m} \prn{\wh H}^{-1} \sum_{z \in u} \grad f(\wh w, z)} \leq  \frac{2 M m^2 L^2}{\lambda^3 n^2}. 
\end{align*}
Using the relation in \pref{eq:dp_guarantee1} and the fact that $\wh w' = \bar{w}$ in the above, we get that 
\begin{align*}
\nrm{\bar{w} - \bar{w}'} \leq \frac{2 M m^2 L^2}{\lambda^3 n^2} \rdef{} \gamma.   \numberthis \label{eq:dp_guarantee2} 
\end{align*} 
Finally, the points $\wt w$ and $\wt w'$ are computed as $\wt w = \bar{w} + \nu$ and $\wt w' = \bar{w}' + \nu$, where the noise $\nu \sim \cN(0, \sigma^2 \bbI_d)$ where $\sigma = \sqrt{2 \ln(\frac{1.25}{\delta})} \cdot \frac{\gamma}{\epsilon}$. Thus, following the same proof as \citet[Theorem A.1]{DworkR14}, with the bound \pref{eq:dp_guarantee2}, we get that for any set $W$, 
\begin{align*}
	\Pr \prn*{ \wt w \in W } &\leq e^\epsilon \Pr \prn*{ \wt w' \in W } + \delta, 
\end{align*}
and that 
\begin{align*}
	\Pr \prn*{ \wt w' \in W } &\leq e^{\epsilon} \Pr \prn*{ \wt w \in W } + \delta, 
\end{align*} which is our desired unlearning guarantee. 
\end{proof}

We next give a bound on the suboptimality with respect to the population loss $F$ for the returned points $\wh w$ and $\wt w$. 
\begin{lemma}[Learning guarantee for $A_{sc}$] 
\label{lem:learning_guarantee__sc} 
For any distribution $\cD$, the output $\wh w$ of running \pref{alg:learningalg_rerm_sco} on the dataset $S \sim \cD^n$ satisfies 
\begin{align*} 
	\En_{S \sim \cD^{n}} \brk{ F(\wh w) - F^*} \leq \frac{4 L^2}{\lambda n}, 
\end{align*} where $F^*$ denotes $\min_{w \in \cW} F(w)$. 
\end{lemma} 
\begin{proof} We note that the point $\wh w$ is given by the empirical risk minimizer on the dataset $S$, i.e. 
\begin{align*}
\wh w = \argmin_{w} \frac{1}{n} \sum_{z \in  S} f(w, z). 
\end{align*}
Since the function $f(w, z)$ is $\lambda$-strongly convex and $L$-Lipschitz, the desired performance guarantee for the ERM point follows from \pref{lem:rerm_works_sc} in the Appendix. 
\end{proof}

The output $\wt w$ of the learning algorithm $\bar{A}_{sc}$ satisfies the following performance guarantee. 
\begin{lemma} 
\label{lem:unlearning_guarantee__sc}
For any dataset $S$, output $\wh w$ of $A_{sc}(S)$ and set $U$ of $m$ delete requests, the point $\wt w$ returned by \pref{alg:unlearningalg_rerm_sco}  satisfies 
\begin{align*}
	\En \brk{F(\wt w) - F^*} = O\prn[\Big]{\frac{ \sqrt{d} M m^2 L^3}{\lambda^3 n^2 \epsilon} \sqrt{\ln\prn[\big]{1/\delta}} + \frac{4mL^2}{\lambda n}}, 
\end{align*} where the expectation above is taken with respect to the dataset $S$ and noise $\nu$. 
\end{lemma} 
\begin{proof} We recall that  
\begin{align*}
\wt w = \wh w +  \frac{1}{n - m} \prn{\wh H}^{-1} \sum_{z \in u} \grad f(\wh w, z) +  \nu,  \numberthis \label{eq:unlearning_guarantee__sc}
\end{align*}
where the vector $\nu \in \bbR^d$ is drawn independently from $\cN(0, \sigma^2 \bbI_d)$ with $\sigma$ given by $\sqrt{2 \ln(\frac{1.25}{\delta})} \cdot \frac{2 M m^2 L^2}{\lambda^3 n^2 \epsilon}$. Thus, 
\arxiv{\begin{align*}
\En \brk*{F(\wt w) - F(w^*)} &= \En \brk*{F(\wt w) - F(\wh w) + F(\wh w) - F(w^*)} \\ 
&= \En \brk*{F(\wt w) - F(\wh w)} + \En \brk*{ F(\wh w) - F(w^*)} \leq \En \brk*{L \nrm*{ \wt w - \wh w}} + \frac{4 L^2}{\lambda n},   \numberthis \label{eq:unlearning_guarantee__sc2}
\end{align*}}
\icml{\begin{align*}
 \hspace{0.5in} & \hspace{-0.5in} \En \brk*{F(\wt w) - F(w^*)} \\ 
&= \En \brk*{F(\wt w) - F(\wh w) + F(\wh w) - F(w^*)} \\ 
&= \En \brk*{F(\wt w) - F(\wh w)} + \En \brk*{ F(\wh w) - F(w^*)} \\ 
&\leq \En \brk*{L \nrm*{ \wt w - \wh w}} + \frac{4 L^2}{\lambda n},   \numberthis \label{eq:unlearning_guarantee__sc2}
\end{align*}} where the inequality in the last line follows from the fact that the function $F = \En \brk*{f(w, z)}$ is $L$-Lipschitz, and by using \pref{lem:learning_guarantee__sc}. Further, from the relation in \pref{eq:unlearning_guarantee__sc}, we have that 
\arxiv{\begin{align*}
\En \brk*{\nrm{\wt w - \wh w}} &= \En \brk{\nrm{  \frac{1}{n - m} \prn{\wh H}^{-1} \sum_{z \in U} \grad f(\wh w, z) + \nu }} \\
&\overleq{\proman{1}} \En \brk{ \sum_{z \in U} \nrm{  \frac{1}{n - m} \prn{\wh H }^{-1} \grad f(\wh w, z)}} + \En \brk*{\nrm{\nu}} \\
&\overleq{\proman{2}} \sum_{z \in U} \frac{1}{(n - m) \lambda} \En \brk{\nrm{ \grad f(\wh w, z) }}  + \sqrt{ \En \brk*{\nrm{\nu}^2}}, 
\end{align*}} 
\icml{\begin{align*}
& \En \brk*{\nrm{\wt w - \wh w}} \\ 
&= \En \brk{\nrm{  \frac{1}{n - m} \prn{\wh H}^{-1} \sum_{z \in U} \grad f(\wh w, z) + \nu }} \\
&\overleq{\proman{1}} \En \brk{ \sum_{z \in U} \nrm{  \frac{1}{n - m} \prn{\wh H }^{-1} \grad f(\wh w, z)}} + \En \brk*{\nrm{\nu}} \\
&\overleq{\proman{2}} \sum_{z \in U} \frac{1}{(n - m) \lambda} \En \brk{\nrm{ \grad f(\wh w, z) }}  + \sqrt{ \En \brk*{\nrm{\nu}^2}}, 
\end{align*}} where the inequality in $\proman{1}$ follows from an application of the triangle inequality, and the inequality $\proman{2}$ holds because the function $F(w)$ is $\lambda$-strongly convex which implies that $\grad^2 F(\wh w) \succcurlyeq \lambda \bbI_d$, and by an application of Jensen's inequality to bound $\En \brk*{\nrm{\nu}}$. Next, using the fact that the vector $\nu \sim \cN(0, \sigma^2 \bbI_d)$, we get that
\begin{align*}
 \En \brk*{\nrm{\wt w - \wh w}} 
&\leq \frac{1}{(n - m) \lambda} \En \brk{\sum_{z \in U} \nrm{  \grad f(\wh w, z) }}  + \sqrt{d} \sigma \\ 
&\leq \frac{m L}{(n - m) \lambda} + \sqrt{d} \sigma, 
\end{align*} where the last line holds because $f(w, z)$ is $L$-Lipschitz. 
Using the above bound in \pref{eq:unlearning_guarantee__sc2}, we get  
\begin{align*}
\En \brk*{F(\wt w) - F(w^*)} &\leq \frac{mL^2}{(n-m) \lambda} + \sqrt{d} \sigma L + \frac{4L^2}{\lambda n}. 
\end{align*}
Our final guarantee follows by plugging in the value of $\sigma$ and using the fact that $n = \Omega(m)$. 
\end{proof} 

\noindent

The above excess risk guarantees for the output of algorithms $A_{sc}$ and $\bar{A}_{sc}$ gives a lower bound on the number of samples $m$ that can be deleted (deletion capacity), while still ensuring the desired excess risk guarantee,  for strongly convex loss functions $f(w,  z)$. 

\begin{proof}[Proof of \pref{thm:main} when $f$ is strongly convex.] 
\pref{lem:dp_guarantee} implies that the learning algorithm $A_{sc}$ and the unlearning algorithm $\bar{A}_{sc}$ are $(\epsilon, \delta)$-forgetting. Furthermore, as a consequence of \pref{lem:unlearning_guarantee__sc}, we see that the number of samples $m$ that can be deleted from the set $S$ (with size $n$) while retaining an excess risk guarantee of 0.01 is given by:
    \[ 
m^{A, \bar{A}}_{\epsilon, \delta}(d, n) \geq c \cdot \frac{n \sqrt{\epsilon}}{\prn*{d\log(1/\delta)}^{1/4}}, 
    \] 
where the constant $c$ depends on the constants $M, K$ and $\lambda$ for the function $f$.
\end{proof} 

\paragraph{Memory requirements.}
We note that the data statistic $T(S)$ that is passed as an input to the unlearning algorithm $\bar{A}_{sc}$ is given by 
$T(S) = \crl[\big]{ \grad^2 \wh F(\wh w)}$. Clearly, $T(S)$ needs $O(d^2)$ memory and thus $\abs{T(S)}$ is independent of $n$ or $m$. For many loss function classes, such as generalized linear models \citep{pregibon1984p}, the
Hessian $ \grad^2 \wh F(\wh w)$ has rank at most $n$, and in this
case, the memory required is $\min\crl{nd, d^2}$.

\paragraph{Computational efficiency.}  While the algorithms $A_{sc}$ and $\bar{A}_{sc}$ compute the exact minimizer for the empirical loss, our bounds also hold if instead we compute an $O(1/n^2)$-suboptimal empirical minimizer. When the domain $\cW$ is convex, such a minimizer can be efficiently computed using standard optimization algorithms like stochastic gradient descent (SGD), clipped-SGD, etc.

\subsection{Convex loss} \label{sec:convex_loss} 
We now provide an unlearning algorithm when the loss function $f$ is convex. In this case, we need to make the following additional assumption on the point $w^*$, which denotes the minimizer of the population loss $F(w) = \En_{z \sim \cD} \brk*{f(w, z)}$. 

\begin{assumption} \label{ass:w_assumption} Any point $w^* \in \argmin_{w \in \cW} F(w)$ satisfies $\nrm{w^*} \leq B$. 
\end{assumption}

Our unlearning algorithms in this case are based on reductions to the strongly convex setting. For the convex function $f(\cdot, z)$, define the function $\wt f(\cdot, z)$ as 
\begin{align*}
\wt f(w, z) = f(w, z) + \frac{\lambda}{2} \nrm*{w}^2. 
\end{align*} 
The key observation is that the function $\wt f(w, z)$ is $\lambda$-strongly convex, $(L + \lambda \nrm{w})$-Lipschitz, $(H + \lambda)$-smooth and $M$-Hessian Lipschitz, and thus we can run algorithms $A_{sc}$ and $\bar{A}_{sc}$ on the function $\wt f$. 

Our learning and unlearning algorithms in this case, denoted by $A_{c}$ and $\bar{A}_c$, and given in  \pref{alg:learningalg_sco} and \pref{alg:unlearningalg_sco} respectively, simply invoke the algorithms $A_{sc}$ and $\bar{A}_{sc}$  on the function $\wt f$ for an appropriately chosen value of $\lambda$.  We additionally define $\wt F$ to denote the population loss with respect to the loss function $\wt f$, i.e. $\wt F(w) \ldef{} \En_{z \sim \cD} \brk{\wt f(w, z)}$. Furthermore, throughout this section, we use the notation $A(S; f)$ to denote the fact that the algorithm $A$ is run on the loss function $f$ (similarly for $\bar{A}$), and whenever clear from context, we will drop the argument $f$ from the notation. 

\begin{algorithm}[tb] 
\caption{Learning algorithm ($A_{c}$)}  
\begin{algorithmic}[1] 
   \Require Dataset $S: \crl*{z_i}_{i=1}^{n} \sim \cD^{n}$, loss function: $f$, regularization parameter: $\lambda$. 
   \State Define $$\wt f(w, z) \ldef{ } f(w, z) + \frac{\lambda}{2} \nrm*{w}^2.$$ 
   \State Run the algorithm $A_{sc}$ on the dataset $S$ with loss function $\wt f$.
   \State \textbf{return} $(\wh w, \wt H) \leftarrow A_{sc}(S; \wt f)$, where $\wt H \ldef{} \frac{1}{n} \sum_{z \in S} \wt f(\wh w, z).$ 
\end{algorithmic} 
\label{alg:learningalg_sco}  
\end{algorithm} 

\begin{algorithm}[tb]
\caption{Unlearning algorithm ($\bar{A}_{c}$)} 
\begin{algorithmic}[1] 
   \Require Delete requests: $U = \crl*{z_j}_{j=1}^{m} \subseteq S$, output of $A_{c}$: $\wh w$, additional statistic $T(S): \wt H$, loss function: $f$, regularization parameter: $\lambda$. 
   \State Define $$\wt f(w, z) \ldef{ } f(w, z) + \frac{\lambda}{2} \nrm*{w}^2.$$ 
   \State Run the algorithm $\bar{A}_{sc}$ for the delete request $U$ with input model $\wt w$ and with loss function $\wt f$. 
   \State \textbf{return} $\wt w \leftarrow \bar{A}_{sc}(S, \wh w, T(S); \wt f)$.  
\end{algorithmic} 
\label{alg:unlearningalg_sco}  
\end{algorithm} 


\begin{theorem}[performance guarantee for $A_{c}$]
\label{thm:convex_learning}
For any $\lambda > 0$ and $S \sim \cD^n$, the point $\wh w$ returned by \pref{alg:learningalg_sco} satisfies
\begin{align*}
\En \brk{F(\wh w) - F^*} &\leq \frac{\lambda B^2}{2} +  \frac{16 L^2}{\lambda n}.  
\end{align*}
\end{theorem}
\begin{proof} First, note that an application of \pref{lem:w_bounded_convex} (stated in the Appendix) implies that for any datatset $S$, the empirical minimizer $\wh w$ (returned by $A_c$) satisfies: $\nrm*{\wh w} \leq \frac{L}{\lambda}$. Thus, our domain of interest is $\cW \ldef{} \crl{w \mid \nrm{w} \leq \frac{L}{\lambda}}$. Over the set $\cW$, the function $\wt f$ if $2L$-Lipschitz, and thus, an application of \pref{lem:learning_guarantee__sc}  implies that the returned point $\wh w$ satisfies 
\begin{align*}
\En \brk{\wt F(\wh w)} &\leq \wt F(\wt w^*) + \frac{16 L^2}{\lambda n}, 
\end{align*} where $\wt w^*$ denotes the minimizer of $\wt F(w)$. We can further upper bound the right hand side above as 
\begin{align*}
\En \brk{\wt F(\wh w)} &\leq \wt F(w^*) + \frac{16 L^2}{\lambda n}, 
\end{align*}
where $w^*$ denotes the minimizer of the population loss $F(w)$. Plugging in the form of the function $\wt F(w)$  in the above, we get  
\begin{align*}
\En \brk*{F(\wh w)} &\leq F(w^*) + \frac{\lambda}{2} \nrm*{w^*}^2 +  \frac{16 L^2}{\lambda n} \\
			   &\leq  F(w^*) + \frac{\lambda B^2}{2} +  \frac{16 L^2}{\lambda n}, 
\end{align*} where the last line holds due to \pref{ass:w_assumption}. 
\end{proof}

\begin{theorem}[performance guarantee for $\bar{A}_{c}$] \label{thm:convex_unlearning} 
For any $\lambda > 0$, dataset $S \sim \cD^n$, output $\wh w$ of $A_{c}(S)$ and set $U$ of $m$ delete requests, the point $\wt w$ returned by \pref{alg:unlearningalg_sco} satisfies 
\arxiv{\begin{align*} 
\En \brk{ F(\wh w)- F^*} &= O\Big( \frac{\lambda B^2}{2} +  \frac{\sqrt{d} M m^2 L^3}{\lambda^3 n^2 \epsilon} \sqrt{\ln\prn{1/\delta}} + \frac{m L^2}{\lambda n} \Big). 
\end{align*}} 
\icml{\begin{align*}
\En \brk{ F(\wh w)- F^*} &= O\Big( \frac{\lambda B^2}{2} +  \frac{\sqrt{d} M m^2 L^3}{\lambda^3 n^2 \epsilon} \sqrt{\ln\prn{1/\delta}} \\ 
& \qquad \qquad \quad + \frac{m L^2}{\lambda n} \Big). 
\end{align*}} 
\end{theorem} 
\begin{proof} Let $w^* \in \argmin_{w} F(w)$. We note that  
\arxiv{\begin{align*}
\En \brk*{F(\wt w) - F(w^*)} &= \En \brk*{F(\wt w) - F(\wh w) + F(\wh w) - F(w^*)} \\ 
&= \En \brk*{F(\wt w) - F(\wh w)} + \En \brk*{ F(\wh w) - F(w^*)} \\ 
&\leq \En \brk*{L \nrm*{ \wt w - \wh w}} + \En \brk*{ F(\wh w) - F(w^*)},   \numberthis \label{eq:unlearning_convex_sc2} 
\end{align*}}
\icml{\begin{align*} 
 \hspace{0.5in} & \hspace{-0.5in} \En \brk*{F(\wt w) - F(w^*)} \\ 
&= \En \brk*{F(\wt w) - F(\wh w) + F(\wh w) - F(w^*)} \\ 
&= \En \brk*{F(\wt w) - F(\wh w)} + \En \brk*{ F(\wh w) - F(w^*)} \\ 
&\leq \En \brk*{L \nrm*{ \wt w - \wh w}} + \En \brk*{ F(\wh w) - F(w^*)},   \numberthis \label{eq:unlearning_convex_sc2}
\end{align*}} where the inequality in the last line holds because the loss function $f(w, z)$, and thus the function $F(w)$, is $L$-Lipschitz. We next note that $\bar{A}_{c}$ computes the point $\wt w$ by running the algorithm $\bar{A}_{sc}$ with inputs $U$, $\wh w$ on the loss function $\wh f$. Thus, we have that 
\begin{align*}
 \hspace{0.3in} & \hspace{-0.3in} \En \brk*{\nrm{\wt w - \wh w}} = \En \brk[\Big]{\nrm[\Big]{  \frac{1}{n - m} \prn{\wh H}^{-1} \sum_{z \in U} \grad \wt f(\wh w, z) + \nu }}, 
\end{align*} where $\wh H \ldef{} \frac{1}{n -m} \sum_{z \in S \setminus U} \grad^2 \wt f(w, z)$. Since, the function $\wt f$ is $\lambda$-strongly convex, we note that $\wh H  \succcurlyeq \lambda \bbI_d$. Using this fact with the above relation implies 
\begin{align*}
 \En \brk*{\nrm{\wt w - \wh w}} &\leq \frac{1}{\lambda(n -m)} \nrm{ \sum_{z \in U}  \grad \wt f(\wh w, z)} + \En \nrm*{\nu} \\ 
 &\leq \frac{1}{\lambda(n -m)} \sum_{z \in U} \nrm{ \grad \wt f(\wh w, z)} + \En \nrm*{\nu} \leq \frac{2mL}{\lambda(n - m)} +  \sigma,  \numberthis \label{eq:unlearning_convex_sc3}
\end{align*} where the last line follows from the fact that $\nrm*{\wh w} \leq \frac{L}{\lambda}$, and thus $$\nrm{\grad \wt f(\wh w, z)} \leq \nrm*{\grad f(\wh w, z)} + \lambda \nrm{\wh w} \leq 2L.$$ 

Finally, using \pref{eq:unlearning_convex_sc3} and  \pref{thm:convex_learning} in  \pref{eq:unlearning_convex_sc2}, and by plugging in the value of $\sigma$ implies the desired performance guarantee. 
\end{proof} 

\begin{corollary} Suppose we did not have any unlearning requests, and only cared about the performance of the output point $\wh w$ for the learning algorithm $A_c$. Then, setting $\lambda = \frac{L}{B\sqrt{n}}$, the performance guarantee for the point $\wh w$ given in \pref{thm:convex_learning} implies 
\begin{align*}
\En \brk{F(\wh w) - F^*} &\leq \frac{BL}{\sqrt{n}}.  
\end{align*} The above rate is tight for learning with Lipschitz convex losses (see  \citet[Theorem 6.1]{bubeck2014convex}).  
\end{corollary}

\begin{corollary}
\label{corr:corollary2}
Suppose that we have $m$ delete requests and thus care about the performance guarantee of both the point $\wh h$, output of the learning algorithm $A_{c}$, and the point $\wt w$, output of the unlearning algorithm $\bar{A}_{c}$. In this case, we set the regularization parameter $\lambda$ as: 
\begin{align}
\lambda = \max \crl[\Big]{\frac{L}{B} \sqrt{\frac{m}{n}}, \prn[\Big]{{\frac{ \sqrt{d} M m^2 L^3}{B^2 n^2 \epsilon} \sqrt{\ln\prn[\big]{1/\delta}}}}^{1/4}}.
\end{align} 
Plugging the above values of $\lambda$ in \pref{thm:convex_learning} and \pref{thm:convex_unlearning}, we get that 
\begin{align*}
\small \En \brk*{F(\wh w) - F^*} = O\prn[\Big]{c_1\sqrt{\frac{m}{n}} + c_2 \prn[\Big]{\frac{d \log(1/\delta)}{\epsilon^2}}^{1/8} \sqrt{\frac{m}{n}}} \\
\intertext{and}
\small \En \brk*{F(\wt w) - F^*} = O\prn[\Big]{c_1 \sqrt{\frac{m}{n}} + c_2 \prn[\Big]{\frac{d \log(1/\delta)}{\epsilon^2}}^{1/8} \sqrt{\frac{m}{n}}},  
\end{align*} 
where the constant $c_1 \propto BL$ and $c_2 \propto \prn[\Big]{ \frac{M L^3}{B^2} }^{1/4}$. 
\end{corollary} 

\noindent
Finally, the algorithms $A_c$ and $\bar{A}_c$ are $(\epsilon, \delta)$-forgetting, as a consequence of \pref{lem:dp_guarantee}. 
\begin{lemma}[Forgetting guarantee] 
\label{lem:dp_guarantee_convex} For any distribution $\cD$, dataset $S \sim \cD^n$, $U \subseteq S$, the algorithms $A_{c}$ and $\bar{A}_{c}$ satisfy the following guarantees for any set $W \subseteq \bbR^d$, 
\arxiv{\begin{enumerate}[label=(\alph*)]
\item $\Pr \prn{\bar{A}_{c}(U, A_{c}(S), T(S)) \in W} \leq e^\epsilon \Pr \prn{\bar{A}_{c}(\emptyset, A_{c}(S \setminus U), T(S \setminus U)) \in W} + \delta$, and 
\item  $\Pr \prn{\bar{A}_{c}(\emptyset, A_{c}(S \setminus U), T(S\setminus U)) \in W} \leq e^\epsilon \Pr \prn{\bar{A}_{c}(U, A_{c}(S), T(S)) \in W} + \delta$. 
\end{enumerate}  
}
\icml{\begin{enumerate}[label=(\alph*)]
\item $\Pr \prn{\bar{A}_{c}(U, A_{c}(S), T(S)) \in W} $ \\ $\leq e^\epsilon \Pr \prn{\bar{A}_{c}(\emptyset, A_{c}(S \setminus U), T(S \setminus U)) \in W} + \delta$, and 
\item  $\Pr \prn{\bar{A}_{c}(\emptyset, A_{c}(S \setminus U), T(S\setminus U)) \in W}$\\ $\leq e^\epsilon \Pr \prn{\bar{A}_{c}(U, A_{c}(S), T(S)) \in W} + \delta$. 
\end{enumerate}}
\end{lemma}

The above excess risk guarantees for the output of algorithms $A_{c}$ and $\bar{A}_{c}$ gives a lower bound on the number of samples $m$ that can be deleted (deletion capacity), while still ensuring the desired excess risk guarantee,  for convex loss functions $f(w,  z)$. 

\begin{proof}[Proof of \pref{thm:main} when $f$ is convex.] \pref{lem:dp_guarantee_convex} implies that the learning algorithm $A_c$ and the unlearning algorithm $\bar{A}_{c}$ are $(\epsilon, \delta)$-forgetting. Furthermore, as a consequence of \pref{corr:corollary2}, we see that the number of samples $m$ that can be deleted from the set $S$ (with size $n$) while retaining an excess risk guarantee of 0.01 is given by:
    \[ 
m^{A, \bar{A}}_{\epsilon, \delta}(d, n) \geq c \cdot \frac{n \sqrt{\epsilon}}{\prn*{d\log(1/\delta)}^{1/4}}, 
    \]
where the constant $c$ depends on the constants $M, L$ and $B$ for the function $f$.
 \end{proof}

==> project_macros_old.tex <==
% general 

% nn_construction.tex
\newcommand{\nn}[1]{f\prn*{#1}}
\newcommand{\relu}[1]{\brk*{#1}_{+}} 
\newcommand{\hinge}[1]{\floor*{#1}_{+}}
\newcommand{\sfE}{\textsf{E}}
\newcommand{\sfG}{\textsf{G}} 

% component_nonconvex.tex
\let\wt\undefined

\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\R}{\bbR}
\newcommand{\empF}{\hat{F}_{n}}
\newcommand{\popF}{F_{\cD}}

\newcommand{\talpha}{\tilde{\alpha}}
\newcommand{\E}{\displaystyle \mathop{\mathbb{E}}}

\newcommand{\clip}{\textrm{Clip}}
\newcommand{\xerm}{x_{\text{erm}}}
\newcommand{\xaerm}{x_{\text{Aerm}}}
\newcommand{\Emax}{E_{\mathrm{max}}}
\def\prob{\text{Pr}}

% Algorithms
\newcommand{\tw}{\widetilde{w}} 
\newcommand{\ssgd}{$\overline{\text{SGD}}$}
\newcommand{\sgd}{SGD}

% Unknown constants
\newcommand{\cone}{c_1} 

% Unknown probabilities
\newcommand{\pone}{p_1} 

% Oracles
\newcommand{\oracle}{\text{\textsf{O}}} 

% General distribution construction
\newcommand{\tepsilon}{\tilde{\epsilon}}
\newcommand{\bw}{\bar{w}} 



% General symbols
\usepackage{amsmath,graphicx}
\newcommand{\widesim}[2][1.5]{
  \mathrel{\overset{#2}{\scalebox{#1}[1]{$\sim$}}}
}

\newcommand{\iid}{\widesim[2]{\text{i.i.d.}}}

% SGD vs RERM
\newcommand{\convexclass}{\mathscr{D}_c}

% Distributions
\newcommand{\uniform}{\text{Uniform}}
\newcommand{\indicator}[1]{\mb{1}\crl*{#1}}
\newcommand{\incomplete}{\text{\textcolor{red}{incomplete}}} 

% Chaining part 
\newcommand{\ramp}[3]{\text{Ramp}\prn*{#1, #2, #3}} 

